How do Wireless Chains Behave? The Impact of MAC Interactions

In a Multi-hop Wireless Networks (MHWN), packets are routed between source and destination using a chain of intermediate nodes; chains are a fundamental communication structure in MHWNs whose behavior must be understood to enable building effective protocols. The behavior of chains is determined by a number of complex and interdependent processes that arise as the sources of different chain hops compete to transmit their packets on the shared medium. In this paper, we show that MAC level interactions play the primary role in determining the behavior of chains. We evaluate the types of chains that occur based on the MAC interactions between different links using realistic propagation and packet forwarding models. We discover that the presence of destructive interactions, due to different forms of hidden terminals, does not impact the throughput of an isolated chain significantly. However, due to the increased number of retransmissions required, the amount of bandwidth consumed is significantly higher in chains exhibiting destructive interactions, substantially influencing the overall network performance. These results are validated by testbed experiments. We finally study how different types of chains interfere with each other and discover that well behaved chains in terms of self-interference are more resilient to interference from other chains.

==> background.tex <==
%\section{Background}
%In this section, we first describe the physical models and the CSMA based medium access protocols that are used in %wireless networks. We then describe the interactions that are generally observed under such network. 

%\subsection{Physical models}
%The received signal power of a wireless transmission attenuates with distance and various other environmental factors. A packet is captured successfully by the receiver if the signal is received correctly and the packet deconstruction occurs without errors. Several theoretical physical models are used to approximate attenuation and packet capture. The \textit{two-disc physical model} is a simplified model of this operation, where a transmission from a node can be sensed by all the nodes that are within a given Interference Range($R_i$). In the absence of interfering signal, a packet can be received by all the nodes that are within the Communication Range ($R_c$, where $R_c<R_i$). Under this model, packet collisions occur when a node is receiving a packet and an interfering node (that is within a distance of $R_i$ from the node) transmits a signal. Under a more advanced \textit{Signal-to-Interference-Noise (SINR) physical model}, a packet can be captured if the ratio of the received signal and the cumulative interference and noise is above a given threshold. While the above physical models cannot accurately capture realistic propagation, they are used used in a majority of the simulators to abstract the physical layer.

%\subsection{CSMA protocols}
%A majority of the wireless networks use Carrier sense multiple access (CSMA) ~\cite{ref:kleinrock_75_ht} based protocols, such as IEEE 802.11, for medium access. CSMA prevents concurrent packet collisions by dictating a node to sense the channel and transmit only if it is sensed idle. However, the channel state at the receiver is
%not known at the sender which gives to the well-known hidden and exposed terminal problems~\cite{ref:bharghavan_94_macaw}.  To counter these effects, protocols such as IEEE 802.11 Distributed Coordination Function (DCF) uses an aggressive CSMA techniques where the channel must be sensed idle for DCF Inter Frame Spacing (DIFS) number of time-slots before the  packet can be transmitted. Optionally, the standard allows the use Collision Avoidance (CA) techniques like (i) reserving the medium through the exchange of Request-to-Send/Clear-to-Send (RTS-CTS) control packets; and (ii) observing prologned periods of silence to avoid congestion if the packet is assumed to be collided.

%In 802.11 DCF, each node maintains a Contention Window ($\operatorname{CW}$) which is preset to a given value $\operatorname{CW_{min}}$ (default value is 31). A node that needs to send a packet initially chooses a \textit{backoff counter} value which is uniformly distributed integer between $[0,\operatorname{CW}]$. If the channel is observed to be idle for DIFS period, then it starts decrementing the $\operatorname{CW}$. The $\operatorname{CW}$ is frozen upon observing a busy channel and the decrementing continues when the channel is observed idle for DIFS period. It transmits the packet when the $\operatorname{CW}$ reaches zero. A packet collision is detected when the acknowledgement (and CTS in RTS-CTS mode) fails to arrive within a given timeout interval. Upon collision detection, the node observes Binary Exponential Backoff (BEB) by doubling the value if ${CW}$. A maximum value of $\operatorname{CW}$ is set to $\operatorname{CW_{max}}$ (default of 1023).

\subsection{What Factors Determine Chain Behavior?}
\label{sec:determinants}
%\saquib{Need a better title}
Several factors affect the performance of chains.  The most important of these factors are described in this section.
%% most important of these factors are: contention unfairness, pipeline
%% effect, cross chain interference, and interference interactions
%% between links of a chain.

\noindent \textbf{Contention Unfairness:} As nodes in a chain compete
for channel access, the ones in the middle of the chain may contend
with more nodes within the chain than those at the edges. These
middle nodes have a smaller chance to transmit, which results in
longer packet queues, ultimately leading to packet drops. We term this
effect {\em contention unfairness} which affects the overall
performance of the chain and is similar to the {\em flow in the
middle}
problem~\cite{ref:chaudet_flowinmiddle}~\cite{ref:wang_05_model}~\cite{ref:garetto_06_starve}.


\noindent \textbf{MAC level Interactions:} One of the factors that
affects the performance of chains is the {\em types of MAC interaction}
between hops of the chains that do not share a common node.  For example, if the source of one hop is a hidden terminal to the receiver of another, the performance of the chain is significantly influenced.
%% Since
%% these hops are capable of transmitting data simultaneously, their
%% interaction with each other impacts the behavior of the chain.

\noindent \textbf{Pipeline Effect:} In a chain, earlier hops feed data to later ones. As a result, later hops can never transmit more
packets than earlier ones.  This effect has important implications: if
there is an interaction leading to unfairness in favor of later hops,
it cannot be sustained.  On the other hand, unfairness in favor of
earlier hops leads to rate mismatch at intermediate hops and packet
drops in queues.  This effect moderates the impact of hidden terminals
and contention unfairness, preventing unfairness in some cases.

\noindent \textbf{Cross-chain Interference:} Chains do not exist in isolation within a network. Links in a chain can have different interactions with links within other chains affecting the overall performance of the network. The effect of this {\em cross chain interference} is an important factor to consider while characterizing the performance of chains.


Of the factors above, the MAC level interactions play a defining role
in the overall performance of the chain. Contention Unfairness,
Pipelining Effect and Cross-chain interference may exist in all chains
to varying degrees but the MAC interactions significantly influence
the impact that these other effects have.  We show examples of this
behavior in Section~\ref{sec:crosschain}. Thus, the first and most
important step in understanding chains is to understand the occurrence
probability and impact of the different MAC interactions within
chains.


% \noindent \textbf{Link Interactions}
% 
% The state of the channel at the receiver determines whether a reception occurs successfully or not. However, carrier sensing is carried out at the sender in Carrier Sense Multiple Access (CSMA) protocols, which does not accurately reflect the state at the receiver. More precisely, if the receiver channel is busy but the sender channel appears idle, a collision occurs - the hidden terminal problem. Conversely, if the receiver channel is available but the sender channel appears busy, the transmission is unnecessarily deferred - the exposed terminal problem. These problems are known to significantly degrade the performance of CSMA in wireless settings~\cite{ref:tobagi_75_ht}. 
% 
% In addition to these problems, protocol-specific interactions might affect the performance of a link. Detailed interactions between two links in CSMA protocols in general and IEEE 802.11 in particular, have been studied~\cite{ref:garetto_05_twoflow, ref:twoflow_sinr}. Garetto \textit{et al.} capture 5 categories of interactions in a simplified two-disc model of interference~\cite{ref:garetto_05_twoflow}. Razak \textit{et al.} capture 10 categories of basic interactions under SINR model. We summarize the three interaction categories that occur most frequently in chains~\cite{ref:twoflow_sinr}. 
% 
% \begin{figure}
%  \centering
% \includegraphics[scale=0.15]{figs/threeLinkCategories.eps}
% \caption{Categories of link interaction}
% \label{fig:linkInteraction}
% \end{figure}
% \noindent \textbf{1. Senders Connected Symmetric Interference (SCSI or SC):} SCSI includes all scenarios where the sources of the two links can sense each other (Figure~\ref{fig:linkInteraction}(a)). Thus, CSMA prevents senders from concurrent transmissions; and no collisions other than those arising when the two senders start transmission at the same time will occur. Such collisions are unavoidable, and their probability is low due to the randomization of the backoff period. In a  homogeneous network and traffic conditions, the two links fairly share the channel due to CSMA rules. We will henceforth refer to the SCSI interaction as \textit{SC} for simplicity.
% 
% \noindent \textbf{2. Asymmetric Incomplete State (AIS or HT):} The senders are not connected in AIS scenarios and, hence, can transmit concurrently. Each sender has incomplete information about the state at the respective receivers. As shown in Figure~\ref{fig:linkInteraction}(b), an asymmetric interference is observed where a transmission from the one sender $S_1$ causes packet collision at the receiver $D_2$ of the other link. The link $S_1D_1$ is unaffected by signals from $S_2$ to $D_2$. The source $S2$ observes large backoff values due to repeated packet collision and hence the throughput of $S_2D_2$ is significantly affected. For simplicity, we henceforth refer to the AIS interaction as \textit{HT} since it experiences severe Hidden-Terminal effect.
% 
% \noindent \textbf{Hidden Terminal with Capture Effect (HTC):} In this interaction, two links have {\em HT} interaction but the destination with the hidden terminal problem is able to capture its packets from its source under interference from the opposite source. Figure~\ref{fig:linkInteraction}(c) shows one possible placement of nodes with HTC interaction. In this case, although $D_2$ is in interference range of $S_1$, it is able to capture its packets from $S_2$ as long as the packet from $S_2$ arrives at $D_2$ before $S_1$ starts transmission. Recent studies have shown that a node can capture packets if it
% has locked on to the packet before the interfering nodes starts
% transmitting~\cite{ref:liliqiu_interference_model}~\cite{ref:kochut_capture}. If the interfering node starts transmitting first,
% the destination node will lock on to its signal and will not be
% able to decode the packet.
% 
% While other categories have significant differences with these interactions, we have observed in our earlier work that such interactions occur infrequently in chains~\cite{ref:srazak_08_selfInterference}. 

%A number of protocols have been proposed to attempt to reduce the effect of the hidden terminal and exposed terminal %problems. Wu and Li propose using a busy tone channel that is used by the receiver when it is receiving a packet %~\cite{wu-87}. Other sources sense this channel allowing carrier sense based on the receiver position. Karn proposed %the MACA protocol (Multiple Access Collision Avoidance), a predecessor to the current IEEE 802.11 protocol %~\cite{ref:karn_90_maca}. MACA uses short request-to-send (RTS, sent by the sender before transmission) and %clear-to-send (CTS, sent by the receiver if RTS is received correctly and the channel is available) to attempt to %reduce collisions. Potential interferers that receive the RTS or the CTS packet do not transmit for the duration of %the packet. Bhargavan et al’s MACAW protocol improves MACA by adding acknowledgement and retransmission %~\cite{ref:bharghavan_94_macaw}.
%Despite these advances in protocol design, the hidden terminal problem continues to plague CSMA MAC protocols. In %fact, depending on the relative location of the senders and receivers, and other factors such as the MAC protocol, %and the interference model, a number of interaction modalities with distinct behavior occur. Bharghavan et al %identify and discuss several of these cases and propose modifications to the MACAW protocol to address them %individually ~\cite{ref:bharghavan_94_macaw} in a network where the interference range is equal to the reception %range 

==> crossChainResults.tex <==
\section{Single chain results}
\begin{figure}
\begin{center}
\includegraphics[scale=0.5]{figs/single-chain/single.th.eps}
\end{center}
\caption{Single Chain: Throughput study: SCSI chains hardly have any variance. Variance of other two is also very small. Very pridictable self-interference pattern.}
\label{fig:single.th}
\end{figure}

\begin{figure*}
\begin{center}
	\mbox{
	\subfigure[SCSI Chain\label{fig:singleChain.single.scsi.linkTh}]{\includegraphics[scale=0.33]{figs/single-chain/single.scsi.linkTh.eps}}\quad
	\subfigure[NI Chain\label{fig:singleChain.single.ni.linkTh}]{\includegraphics[scale=0.33]{figs/single-chain/single.ni.linkTh.eps}}\quad
	\subfigure[AIS Chain\label{fig:singleChain.single.ais.linkTh}]{\includegraphics[scale=0.33]{figs/single-chain/single.ais.linkTh.eps}}\quad
	}
\end{center}
\caption{Link throughputs: SCSI has very little variance even when viewed at each link. Variance of other two is also low. Pipelining perfect in SCSI chains. Pipelining is bad only at link 1. Everything else is perfect from there. Variance is very low.. signifying that self-interference is very predictable}
\label{fig:singleChain.linkTh}
\end{figure*}

\begin{figure}[ht]
\begin{center}
\includegraphics[scale=0.5]{figs/single-chain/single.htContention.eps}
\end{center}
\caption{Comparison of the lost capacity due to hidden terminals and contention unfairness: The blue bar corresponds to the capacity lost in retransmissions. The red/green bar denotes the capacity lost due to queue drops when there is no hidden termianls. This bar shows the effect of contntion unfairness (i.e. How much capacity is lost since the source could not get chance to transmit the packets it received from previous hop).  We find that contention unfairness is controlled due to pipelining in single chain. (Comments to srazak1: Relatively contention unfairness(SCSI)>contention unfairness(NI)>contention unfairness(AIS). We thought that SCSI should have zero CU while others might have some. Looks like pipelining is controlling some stuff)}
\label{fig:singleChain.htContention}
\end{figure}

\section{Detailed results of cross-chain interactions}
\paragraph{High-level conclusions}
\begin{itemize}
\item Stability to topology variations: Happens mainly in parallel (all cases) chains and single-sink when two flows are almost parallel (0-90 degrees). This is because if the destination nodes (or near-destination nodes) are source-connected with source nodes (or near-source nodes), they might have contention unfairness (and half time hidden terminal drops). [In spite of traffic flowing along the same direction]. So, never get hit from severe contention at the destination! But this is unavoidable to a large extent since sources and destinations are generally fixed and intermediate hops can be altered. Routing: Make sure nodes of high contention does not affect later hops of the route.
\item End-to-End throughput: Hidden terminals cause a huge impact in anti-parallel chains when the source gets constantly bombarded by a high traffic (probably src of other chain). In other cases(and a more generally observed phenomenon), contention fairness affects bottleneck links. If bottle-neck links are near source, then the whole chain dies due to:
\item (A)symmetry in two-chain interactions: Symmetry occurs in anti-parallel chains and single sink (when angle between the chains is near 180 degrees). The two chains almost behave identically due to symmetric interactions (if the self-interfrence effect is the same in both chains). Asymmetry is observed in parallel chains (e.g. scenarios of above point ``Stability in topology variations''). 
\end{itemize}

\paragraph{Discussion topics}
\begin{itemize}
 \item How do we identify contention unfairness? Contention unfairness affects chain more when the sources and hops near the sources are present in the larger MICS and the desintaions are in lower order MICS. This can be seen by diminising number of packets sent (even without HTs)
\end{itemize}

\section{Parallel Chains}
\begin{figure*}
\begin{center}
	\mbox{
        \subfigure[2 SCSI-SCSI-SCSI chains\label{fig:parallel.scsi_scsi}]{\includegraphics[scale=0.2]{figs/x-chain/parallel/parallelChains_SCSI_SCSI.eps}} 
        \quad
	\subfigure[2 AIS-SCSI-SCSI chains\label{fig:parallel.ais_ais}]{\includegraphics[scale=0.2]{figs/x-chain/parallel/parallelChains_AIS_AIS.eps}}
	}
	\mbox{
	\subfigure[One AIS-SCSI-SCSI and one SCSI-SCSI-SCSI chain \label{fig:parallel.ais_scsi}]{\includegraphics[scale=0.2]{figs/x-chain/parallel/parallelChains_AIS_SCSI.eps}}
        }
\end{center}
\caption{Parallel chain set-up}
\label{fig:parallel.setup}
\end{figure*}


\paragraph{Overall Conclusions: Parallel chains}
\begin{itemize}
 \item Stability to topology variations due to asymmetry of destination proximity to opposite source: The chain where the destination node contends with the source node of the other chain, suffers from small topological variations (e.g. chain 1 in SCSI-SCSI, chain 2 in AIS-SCSI and AIS-AIS). This is because if the destination nodes (or near-destination nodes) are source-connected with source nodes (or near-source nodes), they might have contention unfairness (and half time hidden terminal drops). [In spite of traffic flowing along the same direction]. So, never get hit from severe contention at the destination! But this is unavoidable to a large extent since sources and destinations are generally fixed and intermediate hops can be altered. Routing: Make sure nodes of high contention does not affect later hops of the route
 \item End-to-End throughput: Generally, if two chains have similar self-interference interactions (2 SCSI-SCSI-SCSI chains or 2 AIS-SCSI-SCSI chains), then the chain whose source is away from the other chain pumps in more packets, and hence gets more throughput. Refer to the difference of throughput histograms. There is one exception cross-chain interaction. When one chain is AIS-SCSI-SCSI and other one is SCSI-SCSI-SCSI, then AIS gets low throughput even though the source is away. \rednote{What happens when the source of SCSI chain is away in this case?}
 \item Minor: If all chains are SCSI's, then very smooth transition as hop length varies.
 \item Minor: If all chains are SCSI's, then smooth transition as we vary slide distance and distance between the chains
 \item \underline{Interaction between AIS-SCSI-SCSI and SCSI-SCSI-SCSI:} Contention fairness affects SCSI a lot. Good throughput is observed when all the links in the SCSI-SCSI-SCSI chain are in higher order MICS. Otherwise the effect of bottleneck link is high and contention unfairness results. For the AIS chain,
 \item \underline{Overall in parallel chains:} Effect of hidden terminals is not too much different than the ones observed in individual chains (self-interference). However, contention fairness might affect the throughput variations for smaller variations in the topology.
\end{itemize}

\clearpage
\subsubsection{Parallel chains -- Vary hop distance and chain distance}
\begin{figure*}
\begin{center}
	\mbox{
        \subfigure[Chain 1\label{fig:parallel.scsi_scsi.chain1}]{\includegraphics[scale=0.45]{figs/x-chain/parallel/scsi_scsi_thHopChainDist.chain1.eps}} 
        \quad
	\subfigure[Chain 2\label{fig:parallel.scsi_scsi.chain2}]{\includegraphics[scale=0.45]{figs/x-chain/parallel/scsi_scsi_thHopChainDist.chain2.eps}}
        }
\end{center}
\caption{Variation in throughput in parallel chains: 2 SCSI-SCSI-SCSI chains. Altering hop distance and distance between the chains}
\label{fig:parallel.scsi_scsi_hop}
\end{figure*}

\paragraph{Conclusions: Parallel -- Vary hop distance vs. chain distance (Figure~\ref{fig:parallel.scsi_scsi_hop})}
\begin{itemize}
 \item If all chains are SCSI's, then very smooth transition as hop length varies. Its very hard to break an SCSI-SCSI-SCSI. If we want to break the chain, we need a strong interferer (relatively nearer). However, if the interferer is nearer, he is most probably source connected and wont transmit concurrently. \rednote{Verify if this is true for all cases. Most probably it is true}
 \item \underline{Negative conclusion:} SCSI-SCSI-SCSIs are very rare. Each hop can be max at around 125m in qualnet where as it can decently communicate even if the src and dest are over 330m. So why would routing protocol choose such routes with such large number of hops \rednote{The overall throughput is similar to AIS-SCSI-SCSI. But how would NI-SCSI-SCSI look}?
\end{itemize}
\clearpage

\subsubsection{Parallel chains -- Vary slide distance and chain distance -- 2 SCSI chains}
\begin{figure*}
\begin{center}
	\mbox{
        \subfigure[Chain 1\label{fig:parallel.scsi_scsi.chain1}]{\includegraphics[scale=0.45]{figs/x-chain/parallel/scsi_scsi_thSlideChainDist.chain1.eps}} 
        \quad
	\subfigure[Chain 2\label{fig:parallel.scsi_scsi.chain2}]{\includegraphics[scale=0.45]{figs/x-chain/parallel/scsi_scsi_thSlideChainDist.chain2.eps}}
        }
	\mbox{
	\subfigure[(Chain 1 - Chain 2) throughput\label{fig:parallel.scsi_scsi.chain1}]{\includegraphics[scale=0.45]{figs/x-chain/parallel/scsi_scsi_thSlideChainDist.diffTh.eps}} 
        \quad
	\subfigure[Histogram of (Chain 1 - Chain 2) \label{fig:parallel.scsi_scsi.chain2}]{\includegraphics[scale=0.45]{figs/x-chain/parallel/scsi_scsi_thSlideChainDist.diffTh.hist.eps}}
	}
\end{center}
\caption{Variation in throughput in parallel chains: 2 SCSI-SCSI-SCSI chains. Altering sliding distance and distance between the chains}
\label{fig:parallel.scsi_scsi}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel/scsi_scsi_link_ChainDist_1m.eps}
\end{center}
\caption{Parallel chains: Chain Distance=1m: SCSI-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L5-L8).SOME OBSERVATIONS: Chain 2 does not have contention unfairness or HTs (except at slideDist=200 and chainDist=500). But chain 1 has both contention unfairness and HTs. At Slide dist=100m, 200m : L1 has half time drops from L5. This might not be captured under our SINR model (Qualnet and MICS model capture this). Also, all MICS have 1-link, but L1, L5 form a 2-link MICS. So they get more channel share. At slide dist=600m chain dist=1m (the bottom pit of the groove shown in Figure~\ref{fig:scsi_scsi.chain1} chain one has HTs(Half time drops) and contention unfairness. After that (slideDist $>$ 600m) all links of the chain 1 come into higher order MICS (one after another) and hence we observe gradual increase in throughput}
\label{fig:parallel.linkTh.scsi_scsi.chDist.1m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel/scsi_scsi_link_ChainDist_50m.eps}
\end{center}
\caption{Parallel chains: Chain Distance=50m: SCSI-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L5-L8).}
\label{fig:parallel.linkTh.scsi_scsi.chDist.1m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel/scsi_scsi_link_ChainDist_100m.eps}
\end{center}
\caption{Parallel chains: Chain Distance=100m: SCSI-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L5-L8).}
\label{fig:parallel.linkTh.scsi_scsi.chDist.1m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel/scsi_scsi_link_ChainDist_200m.eps}
\end{center}
\caption{Parallel chains: Chain Distance=200m: SCSI-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L5-L8)}
\label{fig:parallel.linkTh.scsi_scsi.chDist.1m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel/scsi_scsi_link_ChainDist_300m.eps}
\end{center}
\caption{Parallel chains: Chain Distance=300m: SCSI-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L5-L8).}
\label{fig:parallel.linkTh.scsi_scsi.chDist.1m}
\end{figure*}
\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel/scsi_scsi_link_ChainDist_400m.eps}
\end{center}
\caption{Parallel chains: Chain Distance=400m: SCSI-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L5-L8).}
\label{fig:parallel.linkTh.scsi_scsi.chDist.1m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel/scsi_scsi_link_ChainDist_500m.eps}
\end{center}
\caption{Parallel chains: Chain Distance=500m: SCSI-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L5-L8).}
\label{fig:parallel.linkTh.scsi_scsi.chDist.1m}
\end{figure*}

\paragraph{Conclusions: Parallel -- Vary slide distance vs. chain distance (Figure~\ref{fig:parallel.scsi_scsi})}
This is a scenario where hop distance is almost maximum for a SCSI-SCSI-SCSI chain (around 125m each hop). We vary chain distance and slide distance.
\begin{itemize}
 \item Some non-monotonicity seen as we vary distances. 1 major depression (groove starting at 600m slide distance and 1m chain dist for chain 1 and 400m slide dist and 1m chain dist for chain 2). But else almost monotonic. \rednote{Why is this? Contention fairness or HTs. Why does it decrease first?  And why does it increase next? (Follow the curve at 1m distance)}
 \item A single chain without cross-chain effects gets around $4x10^5$ bps. We can see that chains do not share the throughput fairly.
 \item Chain 1 suffers because of half time drops and contention unfairness. When both are present, the throughput is worse (e.g. chain 1 chaindist=1m slideDist=600m; chainDist=400m slideDist=400m).
 \item All links of chain 2 (the one that is on the top in Figure~\ref{fig:parallel.setup}) always has fair LINK throughputs too (except for chainDist=500m slideDist=0,100,200). \rednote{What makes MICS of chain 2 evenly distributed in single-order MICS?}
\end{itemize}
\clearpage

\subsubsection{Parallel chains -- Vary hop distance and chain distance -- 2 AIS chains}
\begin{figure*}
\begin{center}
	\mbox{
        \subfigure[Chain 1\label{fig:parallel.ais_ais.chain1}]{\includegraphics[scale=0.45]{figs/x-chain/parallel/ais_ais_thSlideChainDist.chain1.eps}} \quad
	\subfigure[Chain 2\label{fig:parallel.ais_ais.chain2}]{\includegraphics[scale=0.45]{figs/x-chain/parallel/ais_ais_thSlideChainDist.chain2.eps}}
        }
	\mbox{
        \subfigure[(Chain 2 - Chain 1) throughput\label{fig:parallel.ais_ais.diffTh}]{\includegraphics[scale=0.45]{figs/x-chain/parallel/ais_ais_thSlideChainDist.diffTh.eps}} \quad
	\subfigure[Histogram of (Chain 2 - Chain 1) throughput\label{fig:parallel.ais_ais.diffTh.hist}]{\includegraphics[scale=0.45]{figs/x-chain/parallel/ais_ais_thSlideChainDist.diffTh.hist.eps}}
        }
\end{center}
\caption{Variation in throughput in parallel chains: 2 AIS-SCSI-SCSI chains: Altering sliding distance and distance between the chains}
\label{fig:parallel.ais_ais}
\end{figure*}
\clearpage

\subsubsection{Parallel chains -- Vary slide distance and chain distance -- AIS and SCSI chains}
\begin{figure*}
\begin{center}
	\mbox{
        \subfigure[Chain 1 - AIS-SCSI-SCSI\label{fig:parallel.ais_scsi.chain1}]{\includegraphics[scale=0.45]{figs/x-chain/parallel/ais_scsi_thSlideChainDist.chain1.eps}}
        \quad
	\subfigure[Chain 2 - SCSI-SCSI-SCSI\label{fig:parallel.ais_scsi.chain2}]{\includegraphics[scale=0.45]{figs/x-chain/parallel/ais_scsi_thSlideChainDist.chain2.eps}}
        }
	\mbox{
        \subfigure[(Chain 1 - Chain 2) throughput\label{fig:parallel.ais_scsi.diffTh}]{\includegraphics[scale=0.45]{figs/x-chain/parallel/ais_scsi_thSlideChainDist.diffTh.eps}}
        \quad
	\subfigure[Histogram of (Chain 1 - Chain 2) throughput\label{fig:parallel.ais_scsi.diffTh.hist}]{\includegraphics[scale=0.45]{figs/x-chain/parallel/ais_scsi_thSlideChainDist.diffTh.hist.eps}}
        }
\end{center}
\caption{Variation in throughput in parallel chains: One AIS-SCSI-SCSI chain and one SCSI-SCSI-SCSI chain: Altering sliding distance and distance between the chains}
\label{fig:parallel.ais_scsi}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel/ais_scsi_link_ChainDist_1m.eps}
\end{center}
\caption{Parallel chains: Chain Distance=1m: AIS-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L5-L8). IMP: Cases where AIS has higher throughput than SCSI: See 800m. \textbf{REASON FOR TH DEGRADATION AT 800M:} L7 not transmitting as much as L6. Reasons: Ack from L1 hits L7 (HTs near destination) + contention unfairness for L7. Contention fairness MICS results: Eg. At 600m, All MICS consist of 2 links. At 700m (point of degradation), There is one MICS of 3 links and every other MICS is 2 links + the source link of C2 (L5) is present in that 3 link MICS. We can see that it is transmitting too much than 600m scenario. At 800m (point of degradation), there are 2 MICS with 3-links in it and rest of the MICS contain 2 links. And yet again L5 is present in one of the 3-link MICS. \textit{So can we say that source rate control at higher layers can stabilize this?}. At 900m, there are 3 MICS with 3-links and rest are 2 links. Links L5, L6 and L7 are present are present in 3-Link MICS. So only L-8 has to contend. So, conclusion \textit{We see the trend that as we increase the distance, the number of higher order MICS gets bigger and additional links from second chain are added to higher order MICS. So, SCSI gets more throughput as distance increases (e.g. from 600m-1000m). We see the bottle-neck link of the SCSI chain moving towards destination. Whenever we see this trend, it most probably is contention unfairness}}
\label{fig:parallel.linkTh.chDist.1m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel/ais_scsi_link_ChainDist_50m.eps}
\end{center}
\caption{Parallel chains: Chain Distance=50m: AIS-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L5-L8). IMP: Cases where AIS has higher throughput than SCSI: See 700m, 800m: At 700m: }
\label{fig:parallel.linkTh.chDist.1m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel/ais_scsi_link_ChainDist_100m.eps}
\end{center}
\caption{Parallel chains: Chain Distance=100m: AIS-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L5-L8). IMP: Cases where AIS has higher throughput than SCSI: See 800m}
\label{fig:parallel.linkTh.chDist.1m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel/ais_scsi_link_ChainDist_200m.eps}
\end{center}
\caption{Parallel chains: Chain Distance=200m: AIS-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L5-L8)}
\label{fig:parallel.linkTh.chDist.1m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel/ais_scsi_link_ChainDist_300m.eps}
\end{center}
\caption{Parallel chains: Chain Distance=300m: AIS-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L5-L8). IMP: Cases where AIS has higher throughput than SCSI: See 700m}
\label{fig:parallel.linkTh.chDist.1m}
\end{figure*}
\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel/ais_scsi_link_ChainDist_400m.eps}
\end{center}
\caption{Parallel chains: Chain Distance=400m: AIS-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L5-L8). IMP: Cases where AIS has higher throughput than SCSI: See 400,500,600,700m. And lot of HTs for SCSI chain}
\label{fig:parallel.linkTh.chDist.1m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel/ais_scsi_link_ChainDist_500m.eps}
\end{center}
\caption{Parallel chains: Chain Distance=500m: AIS-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L5-L8). IMP: Cases where AIS has higher throughput than SCSI: See 300,400,500m}
\label{fig:parallel.linkTh.chDist.1m}
\end{figure*}
\clearpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Anti-parallel Chains}
\begin{figure*}
\begin{center}
	\mbox{
        \subfigure[2 SCSI-SCSI-SCSI chains\label{fig:parallel.against.scsi_scsi}]{\includegraphics[scale=0.2]{figs/x-chain/parallel-against/parallelAgainstChains_SCSI_SCSI.eps}} 
        \quad
	\subfigure[2 AIS-SCSI-SCSI chains\label{fig:parallel.against.ais_ais}]{\includegraphics[scale=0.2]{figs/x-chain/parallel-against/parallelAgainstChains_AIS_AIS.eps}}
	}
	\mbox{
	\subfigure[One AIS-SCSI-SCSI and one SCSI-SCSI-SCSI chain \label{fig:parallel.against.ais_scsi}]{\includegraphics[scale=0.2]{figs/x-chain/parallel-against/parallelAgainstChains_AIS_SCSI.eps}}
        }
\end{center}
\caption{Anti-parallel chain set-up}
\label{fig:parallel.against.setup}
\end{figure*}

\paragraph{Conclusions: Anti-parallel chains}
\begin{itemize}
 \item More symmetric results than parallel chains, i.e. Chain 1 and chain 2 have similar characteristics if they have the same self-interference pattern. Even the link level throughputs have symmetry. This is obvious because of the topology and traffic direction.
 \item Topology variations: Happens too much 2 SCSI chains and AIS-SCSI chains. But it is smooth in AIS-AIS chains. Reason:
 \item
\end{itemize}

\subsubsection{Anti-parallel chains -- Vary hop distance and chain distance -- 2 SCSI chains}
\begin{figure*}
\begin{center}
	\mbox{
        \subfigure[Chain 1\label{fig:parallel.against.scsi_scsi.chain1}]{\includegraphics[scale=0.45]{figs/x-chain/parallel-against/scsi_scsi_thHopChainDist.chain1.eps}} \quad
	\subfigure[Chain 2\label{fig:parallel.against.scsi_scsi.chain2}]{\includegraphics[scale=0.45]{figs/x-chain/parallel-against/scsi_scsi_thHopChainDist.chain2.eps}}
        }
\end{center}
\caption{Variation in throughput in anti-parallel chains: 2 SCSI-SCSI-SCSI chains. Altering hop distance and distance between the chains}
\label{fig:parallel.against.scsi_scsi}
\end{figure*}

\subsubsection{Anti-parallel chains -- Vary slide distance and chain distance -- 2 SCSI chains}
\begin{figure*}
\begin{center}
	\mbox{
        \subfigure[Chain 1\label{fig:parallel.against.slide.scsi_scsi.chain1}]{\includegraphics[scale=0.45]{figs/x-chain/parallel-against/scsi_scsi_thSlideChainDist.chain1.eps}} 
        \quad
	\subfigure[Chain 2\label{fig:parallel.against.slide.scsi_scsi.chain2}]{\includegraphics[scale=0.45]{figs/x-chain/parallel-against/scsi_scsi_thSlideChainDist.chain2.eps}}
        }
\end{center}
\caption{Variation in throughput in anti-parallel chains: 2 SCSI-SCSI-SCSI chains. Altering sliding distance and distance between the chains}
\label{fig:parallel.against.slide.scsi_scsi}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel-against/scsi_scsi_link_ChainDist_1m.eps}
\end{center}
\caption{Anti-parallel chains: Chain Distance=1m: SCSI-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L5-L8)}
\label{fig:parallel.against.scsi_scsi.linkTh.chDist.1m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel-against/scsi_scsi_link_ChainDist_50m.eps}
\end{center}
\caption{Anti-parallel chains: Chain Distance=50m: SCSI-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L5-L8)}
\label{fig:parallel.against.scsi_scsi.linkTh.chDist.50m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel-against/scsi_scsi_link_ChainDist_100m.eps}
\end{center}
\caption{Anti-parallel chains: Chain Distance=100m: SCSI-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L5-L8)}
\label{fig:parallel.against.scsi_scsi.linkTh.chDist.100m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel-against/scsi_scsi_link_ChainDist_200m.eps}
\end{center}
\caption{Anti-parallel chains: Chain Distance=200m: SCSI-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L5-L8)}
\label{fig:parallel.against.scsi_scsi.linkTh.chDist.200m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel-against/scsi_scsi_link_ChainDist_300m.eps}
\end{center}
\caption{Anti-parallel chains: Chain Distance=300m: SCSI-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L5-L8). Half-time drops for L1 of C1 from L1 of C2 and symmetric effect (L1 of C2 from L1 of C1)}
\label{fig:parallel.against.scsi_scsi.linkTh.chDist.300m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel-against/scsi_scsi_link_ChainDist_400m.eps}
\end{center}
\caption{Anti-parallel chains: Chain Distance=400m: SCSI-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L5-L8)}
\label{fig:parallel.against.scsi_scsi.linkTh.chDist.400m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel-against/scsi_scsi_link_ChainDist_500m.eps}
\end{center}
\caption{Anti-parallel chains: Chain Distance=500m: SCSI-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L5-L8): \textbf{NICE::::Reason for the bottleneck drop at L2 at slideDist=50m,100m:} The scenario consists of all 2 link MICS, except thatone MICS has just one link (L2). L2 is not present in any other MICS. So it becomes the bottle-neck due to contention unfairness. Now, why is L6 the bottleneck of other chain? L6 is present with L4 in one 2-link MICS. Since L4 gets hardly any traffic (because L2 is the bottleneck), it does not aid in competing with L4. Hence, for all practical reasons, L4 is virtually single link MICS. Hence it becomes the bottleneck for chain 2! So sources, which are present in the 2-link MICS get all the share. Others, practically in a single-link MICS starve. QED. \textbf{Now REASON FOR balanced throughputs when slideDist=200m:}All 2-link MICS. L2 and L8. Traffic is smooth across all hops (except for the AIS for L1 from L4)}
\label{fig:parallel.against.scsi_scsi.linkTh.chDist.500m}
\end{figure*}
\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Anti-parallel chains -- Vary slide distance and chain distance -- 2 AIS chains}
\paragraph{Conclusions:}
\begin{itemize}
 \item Unlike two-SCSI anti-parallel chains, this is highly asymmetric. The chain 1 almost is ruined and chain 2 enjoys fair throughput (especially when chainDists are small, eg. 1m chainDist and 0m slideDist). This is because L4 of C1 and L1 of C2 are placed right on top of each other and both cause AIS to L1 of C1. Since the source of C2 causes AIS to source of C1, throughput of C1 is decimated.
  \item Lot of hidden terminal effects seen in this scenario. 
  \item Smoothness of the curve: For chain 1, as we move the chain 2 away from the L1 of C1, then the hidden terminal effect gradually gets lower (since instead of the high-traffic source of C2 causing HT on L1, other low-traffic nodes cause HTs. For chain 2: As we move away from C1, we know that C1 gets a little better share of throughput. and then normal channel sharing (contention) takes place and C2 stabilizes gradually.
\end{itemize}

\begin{figure*}
\begin{center}
	\mbox{
        \subfigure[Chain 1\label{fig:parallel.against.ais_ais.chain1}]{\includegraphics[scale=0.45]{figs/x-chain/parallel-against/ais_ais_thSlideChainDist.chain1.eps}} 
        \quad
	\subfigure[Chain 2\label{fig:parallel.against.ais_ais.chain2}]{\includegraphics[scale=0.45]{figs/x-chain/parallel-against/ais_ais_thSlideChainDist.chain2.eps}}
        }
\end{center}
\caption{Variation in throughput in anti-parallel chains: 2 AIS-SCSI-SCSI chains: Altering sliding distance and distance between the chains}
\label{fig:parallel.against.ais_ais}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel-against/ais_ais_link_ChainDist_1m.eps}
\end{center}
\caption{Anti-parallel chains: Chain Distance=1m: AIS-SCSI-SCSI(L1-L4) and AIS-SCSI-SCSI chain(L5-L8)}
\label{fig:parallel.against.ais_ais.linkTh.chDist.1m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel-against/ais_ais_link_ChainDist_50m.eps}
\end{center}
\caption{Anti-parallel chains: Chain Distance=50m: AIS-SCSI-SCSI(L1-L4) and AIS-SCSI-SCSI chain(L8-L5)}
\label{fig:parallel.against.ais_ais.linkTh.chDist.1m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel-against/ais_ais_link_ChainDist_100m.eps}
\end{center}
\caption{Anti-parallel chains: Chain Distance=100m: AIS-SCSI-SCSI(L1-L4) and AIS-SCSI-SCSI chain(L8-L5)}
\label{fig:parallel.against.ais_ais.linkTh.chDist.1m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel-against/ais_ais_link_ChainDist_200m.eps}
\end{center}
\caption{Anti-parallel chains: Chain Distance=200m: AIS-SCSI-SCSI(L1-L4) and AIS-SCSI-SCSI chain(L8-L5)}
\label{fig:parallel.against.ais_ais.linkTh.chDist.1m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel-against/ais_ais_link_ChainDist_300m.eps}
\end{center}
\caption{Anti-parallel chains: Chain Distance=300m: AIS-SCSI-SCSI(L1-L4) and AIS-SCSI-SCSI chain(L8-L5)}
\label{fig:parallel.against.ais_ais.linkTh.chDist.1m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel-against/ais_ais_link_ChainDist_400m.eps}
\end{center}
\caption{Anti-parallel chains: Chain Distance=400m: AIS-SCSI-SCSI(L1-L4) and AIS-SCSI-SCSI chain(L8-L5)}
\label{fig:parallel.against.ais_ais.linkTh.chDist.1m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel-against/ais_ais_link_ChainDist_500m.eps}
\end{center}
\caption{Anti-parallel chains: Chain Distance=500m: AIS-SCSI-SCSI(L1-L4) and AIS-SCSI-SCSI chain(L8-L5)}
\label{fig:parallel.against.ais_ais.linkTh.chDist.1m}
\end{figure*}
\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Anti-parallel chains -- Vary slide distance and chain distance -- AIS and SCSI chains}
\begin{figure*}
\begin{center}
	\mbox{
        \subfigure[Chain 1 - AIS-SCSI-SCSI\label{fig:parallel.against.ais_scsi.chain1}]{\includegraphics[scale=0.45]{figs/x-chain/parallel-against/ais_scsi_thSlideChainDist.chain1.eps}} 
        \quad
	\subfigure[Chain 2 - SCSI-SCSI-SCSI\label{fig:parallel.against.ais_scsi.chain2}]{\includegraphics[scale=0.45]{figs/x-chain/parallel-against/ais_scsi_thSlideChainDist.chain2.eps}}
        }
\end{center}
\caption{Variation in throughput in anti-parallel chains: One AIS-SCSI-SCSI chain and one SCSI-SCSI-SCSI chain: Altering sliding distance and distance between the chains}
\label{fig:parallel.against.ais_scsi}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel-against/ais_scsi_link_ChainDist_1m.eps}
\end{center}
\caption{Anti-parallel chains: Chain Distance=1m: AIS-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L5-L8)}
\label{fig:parallel.against.linkTh.chDist.1m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel-against/ais_scsi_link_ChainDist_50m.eps}
\end{center}
\caption{Anti-parallel chains: Chain Distance=50m: AIS-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L8-L5)}
\label{fig:parallel.against.linkTh.chDist.1m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel-against/ais_scsi_link_ChainDist_100m.eps}
\end{center}
\caption{Anti-parallel chains: Chain Distance=100m: AIS-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L8-L5)}
\label{fig:parallel.against.linkTh.chDist.1m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel-against/ais_scsi_link_ChainDist_200m.eps}
\end{center}
\caption{Anti-parallel chains: Chain Distance=200m: AIS-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L8-L5)}
\label{fig:parallel.against.linkTh.chDist.1m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel-against/ais_scsi_link_ChainDist_300m.eps}
\end{center}
\caption{Anti-parallel chains: Chain Distance=300m: AIS-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L8-L5)}
\label{fig:parallel.against.linkTh.chDist.1m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel-against/ais_scsi_link_ChainDist_400m.eps}
\end{center}
\caption{Anti-parallel chains: Chain Distance=400m: AIS-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L8-L5)}
\label{fig:parallel.against.linkTh.chDist.1m}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/parallel-against/ais_scsi_link_ChainDist_500m.eps}
\end{center}
\caption{Anti-parallel chains: Chain Distance=500m: AIS-SCSI-SCSI(L1-L4) and SCSI-SCSI-SCSI chain(L8-L5)}
\label{fig:parallel.against.linkTh.chDist.1m}
\end{figure*}
\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Single Sink Chains}
\begin{figure}
\begin{center}
\includegraphics[scale=0.2]{figs/x-chain/singleSink/singleSink.eps}
\end{center}
\caption{Single sink set-up}
\label{fig:singleSink.setup}
\end{figure}

\subsubsection{Single sink chains -- Vary angle of rotation}
\begin{figure*}
\begin{center}
	\mbox{
        \subfigure[2 SCSI-SCSI-SCSI chains\label{fig:singleSink.scsi_scsi.thAngle}]{\includegraphics[scale=0.3]{figs/x-chain/singleSink/scsi_scsi.thAngle.eps}} \quad
	\subfigure[2 AIS-SCSI-SCSI chains\label{fig:singleSink.ais_ais.thAngle}]{\includegraphics[scale=0.3]{figs/x-chain/singleSink/ais_ais.thAngle.eps}} \quad
	\subfigure[One AIS-SCSI-SCSI and one SCSI-SCSI-SCSI chain chains\label{fig:singleSink.ais_scsi.thAngle}]{\includegraphics[scale=0.3]{figs/x-chain/singleSink/ais_scsi.thAngle.eps}}
        }
\end{center}
\caption{Single sink model: Througput vs. Angle of rotation}
\label{fig:singleSink.thAngle}
\end{figure*}
\clearpage

\subsubsection{Single sink chains -- Link throughputs}
\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/singleSink/linkTh_scsi_scsi.eps}
\end{center}
\caption{Single sink model: 2 SCSI-SCSI-SCSI chains}
\label{fig:singleSink.linkTh}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/singleSink/linkTh_ais_ais.eps}
\end{center}
\caption{Single sink model: 2 AIS-SCSI-SCSI chains}
\label{fig:singleSink.linkTh}
\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{figs/x-chain/singleSink/linkTh_ais_scsi.eps}
\end{center}
\caption{Single sink model: One AIS-SCSI-SCSI and one SCSI-SCSI-SCSI chain chains}
\label{fig:singleSink.linkTh}
\end{figure*}

\section{Chains with distances taken from Saquib's data}
Points for throughput/fairness (Figure~\ref{fig:randomChains.thFairness})
\begin{itemize}
 \item In throughput graphs (Figure~\ref{fig:randomChains.quar.th}), there not much difference in the throughput between the Lower Quartile, Median and Upper Quartile distances for the 2 SCSI chains, 2 NI Chains and 2 AIS chains. Conclusion: So we dont need to take consider last-hop distance will change throughput (WHEN BOTH CHAINS ARE 4 HOPS) \rednote{Does it change if SCSI}
\end{itemize}

\begin{figure*}
\begin{center}
	\mbox{
        \subfigure[Throughput: Statistical values of hop-distances\label{fig:randomChains.quar.th}]{\includegraphics[scale=0.2]{figs/x-chain/randomChains/quar.th.eps}} \quad
	\subfigure[Throughput: Random picks of hop-distances\label{fig:randomChains.rand.th}]{\includegraphics[scale=0.2]{figs/x-chain/randomChains/rand.th.eps}}}
	\mbox{
        \subfigure[Fairness: Statistical values of hop-distances: Fairness decreases the length of the hast hop increases (Why?). Fairness is best at median i.e. If the length of the last hop is far away from the median (too short or too long), it is susceptible to unfairness\label{fig:randomChains.quar.th}]{\includegraphics[scale=0.2]{figs/x-chain/randomChains/quar.fairness.eps}} \quad
	\subfigure[Fairness: Random picks of hop-distances.Comparing between random and statistical values: Fairness varies more in randomon cases than in the statistical chain (Fig~\ref{fig:randomChains.quar.th}) (in 2 SCSIs, 2 NIs, 2 AISs, SCSI and NI, NI and AIS). Fairness is lesser in random cases than in statistical chains (2 NIs, SCSI and AIS).  \label{fig:randomChains.rand.th}]{\includegraphics[scale=0.2]{figs/x-chain/randomChains/rand.fairness.eps}}}
\end{center}
\caption{Random chain placement: Throughput and fairness study between (a) Individual chains (b) Statistical values of chains. Surprisingly, pretty high fairness values for all chains. Why? (TODO: Look at link throughputs). In fairness 2 SCSI > 2 AIS > 2NIs > NI and AIS > SCSI and NI > SCSI and AIS}
\label{fig:randomChains.thFairness}
\end{figure*}

\begin{figure*}
\begin{center}
	\mbox{
	\subfigure[Median of last hop-distance\label{fig:randomChains.quar.interactions}]{\includegraphics[scale=0.5]{figs/x-chain/randomChains/quar.interactions.prime.eps}} \quad
	\subfigure[Random individual chains\label{fig:randomChains.rand.interactions}]{\includegraphics[scale=0.5]{figs/x-chain/randomChains/rand.interactions.eps}}
	}
\end{center}
\caption{Interaction study: Random chain placement: (1) Not too many cross-chain AISs. (2) Lot of HTC's(NI) popping up (SCSI-SCSI., AIS-AIS, SCSI-AIS}
\label{fig:randomChains.interactions}
\end{figure*}


\begin{figure*}
\begin{center}
	\mbox{
        \subfigure[Lower Quartile of last hop-distance\label{fig:randomChains.quar.scsiLQ.linkTh}]{\includegraphics[scale=0.2]{figs/x-chain/randomChains/quar.scsiLQ.linkTh.eps}} \quad
	\subfigure[Median of last hop-distance\label{fig:randomChains.quar.scsiMedian.linkTh}]{\includegraphics[scale=0.2]{figs/x-chain/randomChains/quar.scsiMedian.linkTh.eps}} \quad
	\subfigure[Upper Quartile of last hop-distance\label{fig:randomChains.quar.scsiUQ.linkTh}]{\includegraphics[scale=0.2]{figs/x-chain/randomChains/quar.scsiUQ.linkTh.eps}} \quad
	\subfigure[Random individual chains\label{fig:randomChains.rand.scsi.linkTh}]{\includegraphics[scale=0.2]{figs/x-chain/randomChains/rand.scsi.linkTh.eps}}
	}
\end{center}
\caption{Link throughputs: Random chain placement: 2 SCSI chains. General conclusion about cross-chain link throughputs: Variance is much larger than single chain case. Shows that the predictablity of performance cannot be nicey generalized like how we did for single chains (Fig~\ref{fig:singleChain.linkTh}). So, no point in trying to generalize when variance is so high. We can just say an average case. Specific about 2 SCSI chains: Pipelining not as good as single chains. Increase in retransmissions due to HTC. Contention unfairness can be slightly seen in later hops of the link. Contention unfairness cannot be seen when we show the average case. However, some cases severely suffer from contention unfairness}
\label{fig:randomChains.2scsis.linkTh}
\end{figure*}

\begin{figure*}
\begin{center}
	\mbox{
        \subfigure[Lower Quartile of last hop-distance\label{fig:randomChains.quar.niLQ.linkTh}]{\includegraphics[scale=0.2]{figs/x-chain/randomChains/quar.scsiLQ.linkTh.eps}} \quad
	\subfigure[Median of last hop-distance\label{fig:randomChains.quar.niMedian.linkTh}]{\includegraphics[scale=0.2]{figs/x-chain/randomChains/quar.scsiMedian.linkTh.eps}} \quad
	\subfigure[Upper Quartile of last hop-distance\label{fig:randomChains.quar.niUQ.linkTh}]{\includegraphics[scale=0.2]{figs/x-chain/randomChains/quar.scsiUQ.linkTh.eps}} \quad
	\subfigure[Random individual chains\label{fig:randomChains.rand.ni.linkTh}]{\includegraphics[scale=0.2]{figs/x-chain/randomChains/rand.ni.linkTh.eps}}
	}
\end{center}
\caption{Link throughputs: Random chain placement: 2 NI chains. }
\label{fig:randomChains.2nis.linkTh}
\end{figure*}

\begin{figure*}
\begin{center}
	\mbox{
        \subfigure[Lower Quartile of last hop-distance\label{fig:randomChains.quar.aisLQ.linkTh}]{\includegraphics[scale=0.2]{figs/x-chain/randomChains/quar.aisLQ.linkTh.eps}} \quad
	\subfigure[Median of last hop-distance\label{fig:randomChains.quar.aisMedian.linkTh}]{\includegraphics[scale=0.2]{figs/x-chain/randomChains/quar.aisMedian.linkTh.eps}} \quad
	\subfigure[Upper Quartile of last hop-distance\label{fig:randomChains.quar.aisUQ.linkTh}]{\includegraphics[scale=0.2]{figs/x-chain/randomChains/quar.aisUQ.linkTh.eps}} \quad
	\subfigure[Random individual chains\label{fig:randomChains.rand.ais.linkTh}]{\includegraphics[scale=0.2]{figs/x-chain/randomChains/rand.ais.linkTh.eps}}
	}
\end{center}
\caption{Link throughputs: Random chain placement: 2 AIS chains.}
\label{fig:randomChains.2aiss.linkTh}
\end{figure*}

\begin{figure*}
\begin{center}
	\mbox{
	\subfigure[Median of last hop-distance\label{fig:randomChains.quar.scsiMedianNiMedian.linkTh}]{\includegraphics[scale=0.2]{figs/x-chain/randomChains/quar.scsiMedianNiMedian.linkTh.eps}} \quad
	\subfigure[Random individual chains\label{fig:randomChains.rand.scsiMedianNiMedian.linkTh}]{\includegraphics[scale=0.2]{figs/x-chain/randomChains/rand.scsiNi.linkTh.eps}}
	}
\end{center}
\caption{Link throughputs: Random chain placement: SCSI and NI chains.}
\label{fig:randomChains.scsiMedianNiMedian.linkTh}
\end{figure*}

\begin{figure*}
\begin{center}
	\mbox{
	\subfigure[Median of last hop-distance\label{fig:randomChains.quar.scsiMedianAisMedian.linkTh}]{\includegraphics[scale=0.2]{figs/x-chain/randomChains/quar.scsiMedianAisMedian.linkTh.eps}} \quad
	\subfigure[Random individual chains\label{fig:randomChains.rand.scsiMedianAisMedian.linkTh}]{\includegraphics[scale=0.2]{figs/x-chain/randomChains/rand.scsiAis.linkTh.eps}}
	}
\end{center}
\caption{Link throughputs: Random chain placement: SCSI and AIS chains.}
\label{fig:randomChains.scsiMedianAisMedian.linkTh}
\end{figure*}

\begin{figure*}
\begin{center}
	\mbox{
	\subfigure[Median of last hop-distance\label{fig:randomChains.quar.niMedianAisMedian.linkTh}]{\includegraphics[scale=0.2]{figs/x-chain/randomChains/quar.niMedianAisMedian.linkTh.eps}} \quad
	\subfigure[Random individual chains\label{fig:randomChains.rand.niMedianAisMedian.linkTh}]{\includegraphics[scale=0.2]{figs/x-chain/randomChains/rand.niAis.linkTh.eps}}
	}
\end{center}
\caption{Link throughputs: Random chain placement: NI and AIS chains.}
\label{fig:randomChains.niMedianAisMedian.linkTh}
\end{figure*}

\begin{figure*}
\begin{center}
	\mbox{
	\subfigure[SCSI-SCSI chain: When C1L1 is not connected to C2L1\label{fig:randomChains.rand.scsi.srcsNotConn.linkTh}]{\includegraphics[scale=0.5]{figs/x-chain/randomChains/rand.scsi.srcsNotConn.linkTh.eps}} \quad
	\subfigure[SCSI-SCSI chain: When C1L1 is connected to C2L1\label{fig:randomChains.rand.scsi.srcsConn.linkTh}]{\includegraphics[scale=0.5]{figs/x-chain/randomChains/rand.scsi.srcsConn.linkTh.eps}}
	}
	\mbox{
	\subfigure[SCSI-AIS chain: When C1L1 is not connected to C2L1\label{fig:randomChains.rand.scsiAis.srcsNotConn.linkTh}]{\includegraphics[scale=0.5]{figs/x-chain/randomChains/rand.scsiAis.srcsNotConn.linkTh.eps}} \quad
	\subfigure[SCSI-AIS chain: When C1L1 is connected to C2L1\label{fig:randomChains.rand.scsiAis.srcsConn.linkTh}]{\includegraphics[scale=0.5]{figs/x-chain/randomChains/rand.scsiAis.srcsConn.linkTh.eps}}
	}
\end{center}
\caption{Link throughputs: Comparision between SCSI-SCSI chains and SCSI-AIS chains. End throughput does not vary much whether C1L1 is connected or not to C2L1 i.e. if they are not connected, lot of queue drops i.e. contention unfairness. When we compare the throughouts in SCSI-AIS chains, we can see that SCSI is not affected much whereas AIS throughput drops by around 30\%}
\label{fig:randomChains.rand.scsi.scsiAis.srcsConnNotConn}
\end{figure*}

\begin{figure*}
\begin{center}
	\mbox{
	\subfigure[C2L1 does not have any interactions with C1\label{fig:randomChains.rand.scsiAis.C2L1HasNoIntWithC1.linkTh}]{\includegraphics[scale=0.5]{figs/x-chain/randomChains/rand.scsiAis.C2L1HasNoIntWithC1.linkTh.eps}} \quad
	\subfigure[C2L1 has SC with C1\label{fig:randomChains.scsiAis.rand.C2L1HasSCWithC1.linkTh}]{\includegraphics[scale=0.5]{figs/x-chain/randomChains/rand.scsiAis.C2L1HasSCWithC1.linkTh.eps}}
	}
	\mbox{
	\subfigure[C2L1 has Asymmetric capture with C1\label{fig:randomChains.rand.scsiAis.C2L1HasHTWithC1.linkTh}]{\includegraphics[scale=0.5]{figs/x-chain/randomChains/rand.scsiAis.C2L1HasHTWithC1.linkTh.eps}}\quad
	\subfigure[C2L1 has AIS with C1\label{fig:randomChains.rand.scsiAis.C2L1HasAISWithC1.linkTh}]{\includegraphics[scale=0.5]{figs/x-chain/randomChains/rand.scsiAis.C2L1HasAISWithC1.linkTh.eps}}
	}
\end{center}
\caption{Link throughputs: SCSI-AIS chain. When Link 1(L1) of AIS chain(C2) is interacting in various ways with links of SCSI chain(C1). C2L1 (which is the weak link of chain 2) has no intearction with any link in C1 for 35.09\% of the time(60 out of 171 scearnios). In the scenarios where there was some interaction, it was seen that an SC interaction with some link of C1 in 81.98\% (97/(171-60)), an HTC interaction with some link of C1 for 45.95\% (51/(171-60). Extremely high value. half the cases saw HTC!) of the sceanrios and an AIS interaction with some link of C1 for 22.5\% (25/(171-60). High value too). So, AIS has higher chances of being unfair! Especially in the cases where there is an AIS interaction for C2L1 from some link of C1, the link C1L1 has almost 75\% losses (4.5Mbps transmitted and 1.1 Mbps received successfully. Figure~\ref{fig:randomChains.rand.scsiAis.C2L1HasAISWithC1.linkTh})}
\label{fig:randomChains.rand.scsiAis.C2L1WithC1}
\end{figure*}

\begin{figure}[ht]
\begin{center}
\includegraphics[scale=0.5]{figs/x-chain/randomChains/conditionalLinkProbs.eps}
\end{center}
\caption{Conditional interaction probability: What is the probability that a link observes AIS/HTC given that it had AIS or HTC or SC in its chain. It can be seen that links that have weak interactions (having AIS or HTC) under self-interference have relatively high probability of being weak in cross-chain interactions. Links that have only SC interactions under self-interference are much more stable. Occurrence of SIS and Symmetric capture effect (SHTC?) are very rare}
\label{fig:rand.conditionalInteractionProb}
\end{figure}

\begin{figure}[ht]
\begin{center}
\includegraphics[scale=0.25]{figs/x-chain/randomChains/rand.htContention.eps}
\end{center}
\caption{Comparison of the lost capacity due to hidden terminals and contention unfairness: The blue bar corresponds to the capacity lost in retransmissions. The red/green bar denotes the capacity lost due to queue drops when there is no hidden termianls. This bar shows the effect of contntion unfairness (i.e. How much capacity is lost since the source could not get chance to transmit the packets it received from previous hop).  Compare this with Figure~\ref{fig:singleChain.htContention}. We find that contention unfairness was controlled due to pipelining in single chain. Whereas we find that the effect is much more significant in cross-chain interactions. Especially SCSI and NI chains have very high vulneribility to contention unfairness. In general, when larger number of independent links contend, this effect has higher chances. Also there is a lot of variance, signifying that the effect is very case-dependent.}
\label{fig:rand.htContention}
\end{figure}

\section{Structure}
We see interactions in a chain
Motivation: Chains function as fundamental unit in MHWNs and link interactions have been thoroughly studied but how they interact in chain is unclear and is complex.
What do we study:
Self-interference (big umbrella) -- interactions in a single chain
  Classify them based on connectedness, hidden terminals and contention unfairness (link interactions)
  What are the most observed chain configurations? 
  How do they behave in terms of:
	1. Throughput : Misc diversions: (why not delay?) (We have the data for saturated traffic, but delay/jitter for saturated traffic doesnt make sense)
	2. Noise (give a difft name) - through Link throughputs 
	3. Pipelining -- How is the pipelining effect for difft chains

We also discuss the multiple chain scenario wrt
Effect of 

